Measuring the Distances to Asteroids from One Observatory in One Night with Upcoming All-Sky Telescopes

Upcoming telescopes like the Vera Rubin Observatory (VRO) and the Argus Array will image large fractions of the sky multiple times per night yielding numerous Near Earth Object (NEO) discoveries. When asteroids are measured with short observation time windows, the dominant uncertainty in orbit construction is due to distance uncertainty to the NEO. One approach to recover distances is from topocentric parallax, which is a technique that leverages the rotation of the Earth, causing a small but detectable sinusoidal additive signal to the Right Ascension (RA) of the NEO following a period of 1 day. In this paper, we further develop and evaluate this technique to recover distances in as quickly as a single night. We first test the technique on synthetic data of 19 different asteroids ranging from $\sim0.05 \,\text{AU}$ to $\sim2.4 \,\text{AU}$. We modify previous algorithms and quantify the limitations of the method, recovering distances with uncertainties as low as the $\sim1.3\%$ level for more nearby objects ($\lesssim$ 0.3 AU) assuming typical astrometric uncertainties. We then acquire our own observations of two asteroids within a single night with $\sim0.1''$ uncertainties on RA, and we find we are able to recover distances to the $3\%$ level. We forecast likely scenarios with the VRO and the Argus Array with varying levels of astrometric precision and expected pointings per night. Our analysis indicates that distances to NEOs on the scale of $\sim0.5$ AU can be constrained to below the percent level within a single night, depending on spacing of observations from one observatory. In a follow-up paper, we will compare these constraints with synchronous and asynchronous observations from two separate observatories to measure parallax even more efficiently, an exciting and likely possibility over the upcoming decade.

==> keywords.tex <==

\begin{keyword}
Topocentric Parallax, Near Earth Asteroids
\end{keyword}

